Learning Vector Quantized Shape Code for Amodal Blastomere Instance Segmentation

Blastomere instance segmentation is important for analyzing embryos' abnormality. To measure the accurate shapes and sizes of blastomeres, their amodal segmentation is necessary. Amodal instance segmentation aims to recover the complete silhouette of an object even when the object is not fully visible. For each detected object, previous methods directly regress the target mask from input features. However, images of an object under different amounts of occlusion should have the same amodal mask output, which makes it harder to train the regression model. To alleviate the problem, we propose to classify input features into intermediate shape codes and recover complete object shapes from them. First, we pre-train the Vector Quantized Variational Autoencoder (VQ-VAE) model to learn these discrete shape codes from ground truth amodal masks. Then, we incorporate the VQ-VAE model into the amodal instance segmentation pipeline with an additional refinement module. We also detect an occlusion map to integrate occlusion information with a backbone feature. As such, our network faithfully detects bounding boxes of amodal objects. On an internal embryo cell image benchmark, the proposed method outperforms previous state-of-the-art methods. To show generalizability, we show segmentation results on the public KINS natural image benchmark. To examine the learned shape codes and model design choices, we perform ablation studies on a synthetic dataset of simple overlaid shapes. Our method would enable accurate measurement of blastomeres in in vitro fertilization (IVF) clinics, which potentially can increase IVF success rate.

==> 4_4_centerbox.tex <==
\subsection{Bounding Box Adjustment for Amodal Segmentation}\label{subsec:method_centerbox}
\wj{if the bounding box adjustment works well.}
While bounding boxes for inmodal segmentation surround visible parts of objects, ones for amodal segmentation can include opaque areas occluded by other objects. For the segmentation module, therefore, it can be ambiguous to determine which object is the target, as exemplified in Fig.~\ref{fig:centerbox}(a). To tackle this ambiguity, we adjust the bounding box by making its center to be located at the center of visible pixels, as shown in Fig.~\ref{fig:centerbox}(b). By rearranging the bounding boxes, the segmentation module conduct segmentation with the center prior (\ie, a target object should be at the center of a bounding box).



==> fig-tex/fig_centerbox.tex <==
\begin{figure}[t]
    \centering
    \subfigure[Box ambiguity]{
    \includegraphics[height=2.5cm]{./figures/centerbox/centerbox_0303_a.pdf}}%\vspace{-0.15cm}
    \subfigure[Inmodal-centered box]{
    \includegraphics[height=2.5cm]{./figures/centerbox/centerbox_0303_b.pdf}}
    \caption{\textbf{Adjustment of bounding box}. (a) For a given detection box (red box), it can include both target (right car) and overlapping (left car) objects. There is uncertainty in determining which object to segment out. (b) To address this issue, we utilize a bounding box of visible pixels (yellow box). We calculate the distance (left yellow arrow) from the center of the visible pixels to the sides of the amodal bounding box (red box). By expanding the bounding box with the same length to the opposite side, we can obtain a new bounding box (green box), whose center is the center of the visible part of the target object.}
    %\vspace{-0.25cm}
    \label{fig:centerbox}
\end{figure}

==> fig-tex/fig_exp_vqvae_mask.tex <==

\begin{figure}[t]
    \centering
    \subfigure[Codewords without perturbations]{
    \includegraphics[width=0.23\columnwidth]{./figures/vqvae_vis/ori_8.png}
    \includegraphics[width=0.23\columnwidth]{./figures/vqvae_vis/ori_1.png}
    \includegraphics[width=0.23\columnwidth]{./figures/vqvae_vis/ori_2.png}
    \includegraphics[width=0.23\columnwidth]{./figures/vqvae_vis/ori_3.png}}\vspace{-0.15cm}
    \subfigure[Codewords with perturbations]{
    \includegraphics[width=0.23\columnwidth]{./figures/vqvae_vis/per_8.png}
    \includegraphics[width=0.23\columnwidth]{./figures/vqvae_vis/per_1.png}
    \includegraphics[width=0.23\columnwidth]{./figures/vqvae_vis/per_2.png}
    \includegraphics[width=0.23\columnwidth]{./figures/vqvae_vis/per_3.png}}
    \caption{Visualization of the embedding space of masks from KINS dataset~\cite{qi2019amodal}. The varying colors in the left color blocks of the subfigures indicate different indices of words at each location. We encode the mask of an object in (a), and then randomly change four matched words as shown in (b). We obtain masks using the VQ-VAE decoder.\wj{consider removing this.}}
    \label{fig:embedding}
\end{figure}


==> fig-tex/fig_model_init.tex <==

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth,height=1in]{example-image-a}
    \caption{\textbf{init.} We show (a) the object instance, (b) overlay with initial mask, and (c) overlay with the refined mask. The mask refinement component better aligns the mask with object boundary.}
    %\vspace{-0.25cm}
    \label{fig:refine_example}
\end{figure}



==> fig-tex/fig_model_refine.tex <==

\begin{figure}[t]
    \centering
    \subfigure[Initial mask]{\includegraphics[width=0.329\columnwidth]{figures/refinement/42_000044_woRef.pdf}}
    \subfigure[Refined mask]{\includegraphics[width=0.329\columnwidth]{figures/refinement/42_000044_wRef.pdf}}
    \caption{\textbf{Mask Refinement Results.} We show an object instance (a) overlaid with an initial mask, and (b) overlaid with a refined mask. The mask refinement component better aligns the mask with object boundary.}
    %\vspace{-0.25cm}
    \label{fig:refine_example}
\end{figure}



==> tab-tex/tab_model.tex <==
\bgroup
\def\arraystretch{1}%  1 is the default, change whatever you need
\begin{table}[t]
    \vspace{0.2cm}
    \centering
    \caption{IoU and mAP indices of VQ-VAE and VAE in various settings.}
    % \resizebox{\linewidth}{!}{
    % \small
    \begin{tabular}{cccc}%|c|}
    \hline %\hline
    \multicolumn{2}{c}{Setting}& IoU & mAP \\
    \hline
    %\hline
    & $K=4$ &\\
    VQ-VAE & $K=8$ & \\
    & $K=16$ &  \\
    \hline
    & $D=64$ &\\
    VAE & $D=196$ & \\
    & $D=512$ &  \\
    \hline
    \end{tabular}
    % }
    \vspace{0.1cm}
\label{table:ablation}
\end{table}
\egroup

==> tab-tex/tab_occlusion.tex <==
\bgroup
\def\arraystretch{1}%  1 is the default, change whatever you need
\begin{table}[t]
    \vspace{0.5cm}
    \centering
    \caption{Shape completion performance for occluded object masks. 
    %The better result is boldfaced.
    }
    \vspace{0.1cm}
    % \resizebox{0.99\linewidth}{!}{
    % \Large
    \begin{tabular}{lcc}%|c|}
    \hline %\hline
    & FCN~\cite{he2017mask} & Ours\\
    \hline
    %\hline
    Geometry & 0.935& \bf{0.968}\\
    KINS & -& \bf{-}\\
    \hline
    \end{tabular}
    % }
    %\vspace{-0.2cm}
\label{table:occlusion}
\end{table}
\egroup

==> tab-tex/tab_speed.tex <==

\bgroup
\def\arraystretch{1}%  1 is the default, change whatever you need
\begin{table}[t]
    \centering
    \caption{Computational speeds of each component. CP, NMS, MG indicate center prediction, non maximum suppression, and mask generation. SPF is seconds per frame.}
    \resizebox{0.75\columnwidth}{!}{
    \small
    \begin{tabular}{ccccc}%|c|}
    % \hline
    \toprule
    & CP & NMS & MG & Total\\
    % \hline
    \midrule
    Time (SPF)& 0.008 & 0.001 & 0.047 & 0.056\\
    \bottomrule
    % \hline
    \end{tabular}
    }
    %\vspace{-0.2cm}
\label{table:runtime}
\end{table}
\egroup
